Exploiting Event Cameras for Spatio-Temporal Prediction of Fast-Changing Trajectories

This paper investigates trajectory prediction for robotics, to improve the interaction of robots with moving targets, such as catching a bouncing ball. Unexpected, highly-non-linear trajectories cannot easily be predicted with regression-based fitting procedures, therefore we apply state of the art machine learning, specifically based on Long-Short Term Memory (LSTM) architectures. In addition, fast moving targets are better sensed using event cameras, which produce an asynchronous output triggered by spatial change, rather than at fixed temporal intervals as with traditional cameras. We investigate how LSTM models can be adapted for event camera data, and in particular look at the benefit of using asynchronously sampled data.

==> Untitled Folder/discussion.tex <==

\section{Conclusions} % contains discussion and conclusions
\label{sec:conclusions}

We showed that LSTM networks could be adapted for event-based data, integrating the temporal component as an input to deal with asynchronous data. The network was characterised for a bouncing ball tracking task, and it was shown that only a small input window is required to achieve a low error. On the other hand, the output window can be extended for as long as necessary, with the trade-off that the error increases linearly. 

Asynchronous \textit{spatial} sampling outperforms \textit{fixed-rate} sampling and therefore we propose that such a strategy, combined with event cameras, is a promising approach for learning to predict trajectories for robotics tasks. For trajectories with variable speeds, more information can be captured by looking at the change in position with a high-resolution, rather than simply sampling at a high rate. Importantly \textit{spatial} sampling is made possible due to the event cameras, which allow asynchronous trajectory sampling directly triggered by change in the scene.


%In our work, \textit{fixed-rate} sampling was performed on the event camera data, as traditional cameras can suffer from motion blur at high target speeds, leading to errors in target tracking, as shown in Fig.~\ref{fig:bouncingBall}.

% The gradient of the linear increase in error is high enough such that predicting for very long periods in front of the ball is not practical. Depending on the exact constraints of the task, other solutions might be to have the network learn only the final position and time of a single trajectory, rather than the full path of the trajectory, allowing the robot to intercept the ball with the correct motion timing.
% Such a network would allow the robot to intercept the ball with the correct motion timing, but not intercept the ball during the trajectory. Alternatively, directly learning to control the arm of the robot from the visual input~\cite{collaborative-hr-handover-lstm}, could also be an interesting direction with \textit{event cameras}.

This study shows the advantage of spatial sampling in input data using event cameras and in the following visual processing, using asynchronous output events also in computational models such as the tracking, motivating a further quest in the use of event-driven perception coupled with LSTM architectures for fast vision tasks in artificial intelligence and robotics.
Depending on the exact constraints of the task, other solutions might be to have the network learn only the final position and time of a single trajectory, rather than the full path of the trajectory, allowing the robot to intercept the ball with the correct motion timing.
Future work will aim at improving the performance of the hereby presented architecture and evaluating other possible solutions, before moving to the robot control. 

% Such a network would allow the robot to intercept the ball with the correct motion timing, but not intercept the ball during the trajectory. Alternatively, directly learning to control the arm of the robot from the visual input~\cite{collaborative-hr-handover-lstm}, could also be an interesting direction with \textit{event cameras}.

% Such a network would allow the robot to intercept the ball with the correct motion timing, but not intercept the ball during the trajectory. Alternatively, directly learning to control the arm of the robot from the visual input~\cite{collaborative-hr-handover-lstm}, could also be an interesting direction with \textit{event cameras}.


%sampling inherent to event-based camera

%frame-based camera could have other downsides for the tracker.





%Figure~\ref{fig:whole_traj} illustrates a qualitative evaluation of the predictor capabilities over the entire trajectory of a single ball bounce. 
%On the complete trajectory (in blue) recorded from the ATIS camera, are shown the input points (in green) and the respective prediction (in purple) obtained from the Encoder-Decoder model at different time instants.
%The network is continuously queried with new inputs, providing an updated estimate every time. This, along with the low latency guaranteed by the event cameras, allows for a rapidly adaptive predictive system.
%Even though a frame-based camera could still be able to capture meaningful points and output a valid prediction, a system like this has the advantage of not suffering image artifacts - like blur - nor requires long exposure times. In more extreme cases, where very low latencies are required or safety and reliability are strongly needed (as in drones control or autonomous driving), this topic becomes crucial. Every point can be informative and determine the success of the task at hand.
%What we did not address in this paper and will represent a future extension to the work is how many points are needed to have a good prediction, mostly in relation to the temporal dynamics of the task considered. Even with the lower power consumption needed by event cameras, computing a new prediction every time a new point arrives could represent a waste of power and computational resources. A spatial filtering might represent a first solution, as the opposite with time is now not possible having asynchronous data points.
%Another approach could be inspired by \textit{predictive coding}, outputting a new prediction when some predefined conditions occur, like the exceeding of a certain threshold between a past prediction and the current point received. This would allow for a lower number of network queries, and hence resources consumption, that would be triggered only when the motion diverges from the expected one - like the sudden hit of a table and the consequent bounce of the ball. This would be possible thanks to the event camera properties; while, with a frame-based system, everything would be bounded to the fixed rate of the device.



%\section{Conclusions and Future Work} % contains discussion and conclusions
%\label{sec:conclusions}

%The work proposed here wants to represent a pilot study for the development of an event trajectory prediction systems. Exploiting the temporal information associated with their output, event cameras represent an appealing solution for capturing the dynamics of fast-changing movements in an autonomous system's field of view.
%In this paper we addressed the problem of predicting the trajectory of a bouncing ball from the iCub viewpoint, resorting to an ATIS camera placed in the robot eye.
% The spikes generated by the ball motion contribute to the computation of a events centre-of-mass in a user-defined region-of-interest. This point represents the input of a LSTM Encoder-Decoder network, that returns a prediction of what will be the next sequence of spatio-temporal points.
% The dataset creation and the cross-validation process to determine the optimal input and output buffer sizes have been reported in Section~\ref{sec:experiments}, while in Section~\ref{sec:discussion} advantages and drawbacks of the proposed method have been presented and discussed.
%From Section~\ref{sec:experiments} and \ref{sec:discussion}, it comes out that a predictor system can benefit from an event approach thanks to its low latency and dense output trace, allowing for a rapidly adaptive prediction. Time is now an available information that can be inputted as a feature and that can be learned, adapting the estimate provided by the predictor to the task dynamics: short-term information will be provided for fast movements and long-term information will be given for slower ones.
%On the other hand, such dense trajectories seem to not improve the quality of the prediction. A filtering process might be therefore applied to reduce the amount of computation. Further tests are needed in this direction, in order to understand how many points are needed to well characterize a motion dynamics and have a good prediction.
%Future work will also introduce 3D perception by means of a stereo system or using cooperative networks \cite{cooperative_nets} to retrieve depth from events. Subsequently, online testing on the iCub will be carried out, evaluating how prediction horizon, computational time and control latencies affect the interaction.

==> Untitled Folder/experiments.tex <==

\section{Experiments and Results}
\label{sec:experiments}

%=====================================================================
\begin{figure}
  \centering
        % \centering
        \includegraphics[width=\linewidth]{whole_traj.pdf}
        % \caption{}
        % \label{subfig:RMSE_space_wf}
  \caption{Complete example of a ball trajectory (in blue) with pairs of input (in green) and prediction (in purple) at different time instants.}
  \label{fig:whole_traj}
\end{figure}
%=====================================================================







% %=====================================================================
%  \begin{figure}[b]
%   \centering
%         % \begin{subfigure}[!tb]{\linewidth}
%             % \centering
%             \includegraphics[width=\linewidth]{spatial_and_tempora_error_fixedW-OUT_differentW-IN.png}
%             % \caption{}
%             % \label{fig:RMSE_wi}
%         % \end{subfigure}
%         % \begin{subfigure}[!tb]{\linewidth}
%         %     \centering
%         %     \includegraphics[width=\linewidth]{TimeError_different_win.pdf}
%         %     \caption{}
%         %     \label{subfig:RMSE_time_wi}
%         % \end{subfigure}
%   \caption{Spatial and Temporal RMSE for different $w_{in}$ values assuming $w_{out}=35$ points.}
%   \label{fig:RMSE_win}
% \end{figure}
%=====================================================================

% training info
A dataset was collected with 250 individual trajectories of the ball thrown in front of the camera and bouncing 2 or 3 times. The $<x_{b_i},y_{b_i},t_{b_i}>$ output of the tracker module was recorded. For independence to the direction of the trajectory, all datasets were flipped along the x-axis resulting in a total of 500 trajectories. The dataset was split into 470 training trajectories, 20 validation trajectories and 10 test trajectories. A trajectory example is shown in space-time in Fig.~\ref{fig:whole_traj}.

To choose the right Encoder-Decoder architecture, we started with a spatial sub-sampling of $D=2$ pixels and trained several models assuming different values for $w_{in}$ and $w_{out}$. Then, to compare the effect of the two sampling strategies, we chose suitable $F$ values for the \textit{fixed-rate} sampling and $D$ values for the \textit{spatial} sampling, to cover the same time intervals and looked at the test error. 

% To choose the right Encoder-Decoder architecture, we started with a spatial sub-sampling of $D=2$ pixels and, considering $w_{in} \in [2, 6, 10, 15, 20, 25, 30, 40]$ and $w_{out} \in [8, 15, 25, 35, 45, 60]$, performed a hyper-parameters tuning process.

% To compare the effect of sampling strategies, several models were trained with the two strategies. For the \textit{fixed-rate} sampling were chosen time intervals $F \in [5, 10, 15, 20, 25, 33, 50]$ milliseconds; for the \textit{spatial} sampling were chosen delta values $D \in [2, 4, 6, 8, 10, 12]$ pixels.

The Adam optimization algorithm~\cite{adam} was used with a learning rate of 0.01. Dealing with a regression problem, the Mean Squared Error (MSE) was adopted as loss function. No dropout was used and the networks were trained for 200 epochs on batches of size 128.

%=====================================================================
\begin{table}
\centering
\begin{tabular}{|| c| c ||}
\hline
Spatial delta D (pxl) & Mean+STD rate [Hz]\\ 
\hline\hline
-  & 357$\pm$88\\
2  & 182$\pm$44\\
4  & 92$\pm$22\\ 
6  & 63$\pm$14\\
8 & 48$\pm$11\\
10 & 39$\pm$9\\
12 & 33$\pm$7\\
% 30 & 14$\pm$3\\
\hline
\end{tabular}
\caption{Spatial delta sampling values with corresponding computational rate (mean and standard deviation).}
\label{table:samples}
\end{table}
%=====================================================================

 
 \subsection{Sequence-to-Sequence Characterisation}
 
To initially characterise some parameters of the LSTM, the prediction root-mean-square error (RMSE) error was calculated for prediction trajectories, according to trajectory spatial error and temporal error reported in to Fig.~\ref{fig:error_definition}. %The \textit{spatial error} for a single trajectory point is defined as the difference between the estimated pixel coordinate  $< \hat{x_{b_i}},\hat{y_{b_i}} >$ and the ground truth coordinates $< x_{b_i},y_{b_i} >$ at a fixed point in time. In order to perform a comparison, the ground-truth trajectory is interpolated to calculate the position at exact time of a predicted point $t_{b_i}$. On the other hand, the \textit{temporal error} for a point $< \hat{x_{b_i}},\hat{y_{b_i}} >$ represents the difference between its predicted time of occurrence $t_{b_i}$ and the time when the ball actually reached the same position $t_{b_i}$. Again the ground-truth trajectory is interpolated and the closest point on the trajectory is considered. 
The RMSE is the mean error along the entire predicted length, and not only the final position.

The error increases linearly with the output window length $w_{out}$, meant as number of points predicted in a single network interrogation, for both the spatial error and the temporal error, as shown in Fig.~\ref{fig:RMSE_fixed_win}. As the network tries to predict further ahead, the accuracy at which it can do so decreases. As the relationship is linear, there is no optimal point at which the network operates. The choice is therefore application specific, trading off the amount of time ahead that is needed, compared to the highest acceptable error.

The spatial error decreases the more data in the past is used, $w_{in}$. However, after a certain value, there is no real benefit in feeding more points, as shown in Fig.~\ref{fig:RMSE_fixed_wout}. In this case, a systematic operating point could be chosen to achieve the lowest error.

In the following, the output window length $w_{out}$ was set to be 45 and the input window length $w_{in}$ was set to 20.

\subsection{Sampling Strategy Comparison}

%=====================================================================
\begin{figure}
    \centering
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=.8\linewidth]{average_spatial_and_temporal_error_fixedW-IN_differentW-OUT-2.pdf}
        \caption{}
        \label{fig:RMSE_fixed_win}
    \end{subfigure}
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=.8\linewidth]{average_spatial_and_temporal_error_fixedW-OUT_differentW-IN-2.pdf}
        \caption{}
        \label{fig:RMSE_fixed_wout}
    \end{subfigure}
        % \centering
        %\includegraphics[width=\linewidth]{RMSE_different_wout.pdf}
        %\includegraphics[width=\linewidth]{spatial_and_temporal_error_fixedW-IN_differentW-OUT.png}
        % \caption{}
        % \label{subfig:RMSE_space_wf}
  \caption{Spatial and Temporal RMSE for different (a) $w_{out}$ values assuming $w_{in}=20$ and (b) $w_{in}$ values assuming $w_{out}=45$.}
  \label{fig:RMSE_winwout}
 \end{figure}
% %=====================================================================

%=====================================================================
\begin{figure}[t]
  \centering
  \begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=0.9\linewidth]{S-RMSE_different_rates2.pdf}
  \caption{}
  \label{fig:srmse_different_rates}
  \end{subfigure}
  \begin{subfigure}{\linewidth}
  \centering
  \includegraphics[width=0.9\linewidth]{predictor_rate2.pdf}
  \caption{}
  \label{fig:predictor_rate}
  \end{subfigure}
  \caption{The (a) spatial RMSE for fixed-rate and spatial sampling, in which the mean sample rate of time is used to place the spatial sampling, and (b) the sample rate for spatial sampling over time for an example trajectory.}
\end{figure}
%=====================================================================

Secondly, a comparison between sampling strategies was made with respect to the prediction accuracy. Considering an input window of about $~90ms$ and an output window of about $~200ms$ defined by the previous windows length choice, we compare the performance of the two sub-sampling strategies on the same time intervals.

Fig.~\ref{fig:srmse_different_rates} shows the error for both sampling strategies. In order to perform a comparison, the mean sampling rate of the spatial was calculated (after sampling) and used as a comparison point to the fixed-rate sampling. Fixed-rate sampling showed an inverse relationship to error. A low rate results in a high error, and as the rate increases, the error decreases. However, the benefit of increased sample rate beyond 67 Hz is minimal. 

Spatial sampling instead shows a more linear decrease in error with respect to sampling rate. The error reaches a minimum value of 7.52 pixels for a spatial of 2 pixels, compared to a value of 10.08 pixels when using a fixed 200 Hz sampling rate. Importantly, the lower error is also achieved with less processing requirements as the average rate (and hence the total number of calculations) is lower for the 2 pixel spatial sampling.

The reason that the spatial sampling can give a lower error for an identical mean sampling rate is that it gives a varying sample rate in time, over the length of the dataset. In periods of fast and non-linear motion, where fine details are required to correctly trace the motion, the sample rate increases also enabling a more accurate prediction. On the other hand, when the target is moving slowly, the sample rate decreases and processing savings can be achieved. Fig.~\ref{fig:predictor_rate} shows an example sample rate (in time) for the spatial sampling, and it can be seen that for larger spatial deltas the sample rate becomes more constant across the dataset (a flatter profile). For sample rates without much variation, the error is much closer to that of fixed-rate sampling, as shown in Fig.~\ref{fig:srmse_different_rates}. 

%To choose the right values for $w_{in}$ and $w_{out}$ different models have been trained, combining the two parameters in a grid search process. In order to evaluate separately the spatial and temporal prediction error, we have defined sequence-to-sequence error metrics that quantify the error of the predicted sequences in comparison to the ground-truth trajectory. 
%Figure~\ref{fig:error_definition} illustrates how these errors are calculated.
%To compute these two error components, an interpolation process has been applied to retrieve data not directly available from the original sequences, even though the very high resolution of the event cameras would be already enough to have a first approximation of the metrics.




%=====================================================================
% \begin{figure}[tb]
%   \centering
%   \includegraphics[width=\linewidth]{predictor_rate2.png}
%   \caption{Predictor rate.}
%   \label{fig:predictor_rate}
% \end{figure}
%=====================================================================






%The training process optimizes the network weights to reduce the loss function over the whole output sequence. Therefore, we evaluated how the sequence-to-sequence error changes with the number of points ahead we try to predict. Figure~\ref{fig:RMSE_wout} shows that the error increases linearly with the length of the output sequence. For the sake of space, we present here only the case with input sequence $w_{in} = 10$ points, but the same trend has been encountered also in the other cases, meaning that the choice of $w_{out}$ depends only on the error value related to $w_{in}$ and our acceptance threshold. As a compromise between prediction horizon and error, we have chosen $w_{out} = 35$.
%In Figure~\ref{fig:RMSE_wout} it has been reported also the error of a predictive system operating at a fixed rate of $33 ms$. A model has been trained taking in input 2 points and outputting a prediction of 3 points, in order to compare the spatial error of our networks with a model that operates in a frame-based fashion and on a comparable temporal horizon of around 0.1 seconds. It is important to remark that, event if the fixed rate is similar to a frame-based camera, this network takes as input points obtained by subsampling of an original event trajectory, which is not affected by blur. Real frame-based cameras might not be able to catch precisely the ball position because of artifacts, resulting in sparse and noisy trajectory points. 

%With regard to the input buffer, Figure~\ref{fig:RMSE_win} shows how, for the same fixed prediction horizon, the spatial error trend evolves for different values of $w_{in}$. The same for the temporal error is shown in Figure~\ref{fig:RMSE_win}. 
%It comes out that an optimal choice for the input buffer size can be $w_{in}=10$, presenting one of the lowest spatial errors and the lowest temporal error.



==> Untitled Folder/introduction.tex <==

\section{Introduction}
\label{sec:intro}

Predictive capabilities can massively improve the safety and reliability of robots as they interact with the environment. Humans make use of predictive estimates daily, and almost in an unconscious manner, for instance when driving, playing sports or interacting with other people. A similar capability in robots could further allow them to be integrated amongst humans, and be utilised for a wider range of tasks. In addition, forecasting information about the surrounding environment can allow a robot to plan actions in advance, and in a way to compensate for insufficiency in their actuation and movement capabilities. As such, high performance robots will not be limited to robots with high-quality, highly-precise, but costly, actuators and parts.
However, the motion of many things in the environment is not easily predictable with simple extrapolation, as, for example, biological motion can be highly non-linear and sporadic. Patterns still exist in the data, but a simple model may not be sufficient, with the need to resort to data driven learning.
%A fitting example is the use of Long Short-Term Memory networks (LSTM)~\cite{LSTM} when dealing with time series, state-of-the-art architecture for time-dependent tasks thanks to its ability of avoiding vanishing gradient problems. The possible applications are many. In ~\cite{gait-stability-prediction} this type of network has been used in a more general framework to predict the gait stability of elderly people for a robotic walking frame, acting as a fall-risk alarm. The output prediction can also be used as reference signal for control, like in~\cite{lstm-path-planning}, where a LSTM is used as path planner for a mobile robot moving in an unknown environment and relying only on a local map. The same approach is adopted in~\cite{collaborative-hr-handover-lstm} to generate the robot end-effector desired path in response to a human handover motion.
Training neural networks to learn to predict trajectories has been successful in gait stability for fall-risk monitoring~\cite{gait-stability-prediction}, as well as for robot manipulator control~\cite{collaborative-hr-handover-lstm} and path planning~\cite{lstm-path-planning}.
%Successful examples are the works in~\cite{gait-stability-prediction}, ~\cite{lstm-path-planning} and ~\cite{collaborative-hr-handover-lstm}. In ~\cite{gait-stability-prediction} a framework for predicting the gait stability of elderly people is developed as fall-risk alarm for a robotic walking frame. In ~\cite{lstm-path-planning} and ~\cite{collaborative-hr-handover-lstm}, instead, the output prediction serves as reference signal for the robot to control. In the first work the predictor acts as path planner for a mobile robot in unknown environments; in the second one, it generates the robot end-effector desired path in response to a human handover movement.


%=====================================================================
\begin{figure}[!t]
  \centering
        \begin{subfigure}[!tb]{.49\linewidth}
            \centering
            \includegraphics[width=\linewidth]{bouncingBallRBG.png}
            \caption{}
            \label{subfig:bouncingRBG}
        \end{subfigure}
        \begin{subfigure}[!tb]{0.49\linewidth}
            \centering
            \includegraphics[width=\linewidth]{bouncingBallED.png}
            \caption{}
            \label{subfig:bouncingED}
        \end{subfigure}
  \caption{The trajectory of a bouncing ball comparing the sample points for (a) a traditional camera that samples at a fixed-rate in time, and (b) an event camera that samples with a fixed spatial sampling. The event camera output is shown with all the pixel-wise events (in purple) as well as the output of the trajectory tracker (in blue).}
  \label{fig:bouncingBall}
\end{figure}
%=====================================================================

To extend beyond what already exists in the field, we propose the use of \textit{event cameras}~\cite{ATIS}. Specifically, in this paper we analyse possible advantages in combining a classical deep learning strategy for sequence prediction with this type of sensors. Event cameras are a novel paradigm in machine vision that output a single \textit{event} for each pixel, but only when a change in the intensity of light falling on the pixel occurs. This happens when an object is moving in front of the camera, or at points of high contrast (e.g. edges of structure, edges of objects) when the camera itself moves. Such a technology acquires highly-compressed and low-latency (15 $\mu s$~\cite{ATIS}) visual trajectories of moving targets. The biggest conceptual difference when compared to a traditional camera is that an event camera samples a target trajectory based on its change in spatial value, i.e. the sampling of the vision signal is driven by the change in position. We therefore achieve a trajectory with samples at pixel, or sub-pixel, resolution, independently of the speed of the target. A comparison to a traditional camera, which samples at a fixed time period, is shown in Fig.~\ref{fig:bouncingBall}.

Event cameras are suited for dynamic tasks, such as camera pose estimation~\cite{6d0f_camera_relocalization,visual_inertial_odometry}, object tracking~\cite{arren_tracker}, and action recognition~\cite{ed_gesture_recog}. Visual learning has also been performed with event-data for classification~\cite{event-cnn1, event-cnn2}, ego-motion computation~\cite{event-driven_ego-motion}, depth estimation~\cite{event-driven_depth}, and vehicle steering prediction~\cite{event-driven_steering-angle1, ed_steering_prediction}. However, the majority of these works use convolutional neural networks (CNN) that do not inherently represent time, which is a very informative signal for event cameras. 

%Nevertheless, when combining events with architectures like CNN we do not fully exploit the temporal information associated with the data. 

Recurrent Neural Networks (RNN) are designed to handle and learn patterns in sequential data. One of the most important RNN was introduced in 1990 by Elman~\cite{elman}, but, the work suffered from vanishing, exploding gradients~\cite{LSTM}. Long Short-Term Memory networks (LSTM)~\cite{LSTM} overcome this problem and are currently the state-of-the-art in the field of RNNs. 
%In recent years, in the wave of deep learning, LSTM has been imposed as the most used RNN architecture when dealing with sequences. 
The Encoder-Decoder - or Sequence-to-Sequence - model~\cite{seq2seq-text_transl} achieves state of the art results in several fields like Natural Language Processing~\cite{seq2seq-text_transl, seq2seq-speech_recog, seq2seq-image_capt} since it can map input sequences to output ones with different length. An Encoder-Decoder network has been combined also with a \textit{beam search} algorithm for predicting vehicle trajectories~\cite{seq2seq-vehicle_trajs} for self-driving cars. %Investigating the potential for deep-learning using event cameras and LSTM models is a potentially rewarding and unexplored area of research.% Thus, in this work we decided to use the LSTM Encoder-Decoder model for predicting trajectory of a bouncing ball due to its excellent performance and because we can use different length sequences as input and output of the Encoder-Decoder model.

In this paper we investigate the integration of event-data with the LSTM architecture for learning to predict the trajectory of a bouncing ball focusing on the effect of different sampling strategies when combined with the learning architecture: \textit{fixed-rate} sampling, as performed in traditional cameras, compared with \textit{spatial} sampling, as is associated with event cameras. Experiments are performed using the neuromorphic iCub robot~\cite{Bartolozzi2011} equipped with the ATIS~\cite{ATIS} event camera. The ball bounces on a table in front of the robot and the robot, using the observed past ball positions, predicts the future trajectory for a given sequence. %The final goal of such an artificial intelligence is for the robot to decide the best interception strategy with its hand in order to catch the ball. In this case, the temporal component, as well as the spatial positions, become important information, as the robot must select both the space and time at which the interception must occur. Note, in these studies we focus on the prediction-only.

%Vision has become a major source of sensory information for robots, being cheap, passive and giving rich information. The time needed to acquire a single image, however, determines the maximum rate at which the device can operate and, consequently, limits the operating rate of all the other downstream systems. If the environment is moving faster than the camera and processing can handle, the robot can fail its task. On the other hand, if the environment is stationary, standard camera technology acquires multiple frames of redundant, non-changing data. Processing such data is a waste of power and computational resources that could be otherwise used elsewhere. %Conversely, in case of fast changes, the device might not be able to capture the whole dynamics of the latter, failing to respect the Nyquist-Shannon sampling theorem. 
%Standard cameras are therefore only optimal for tasks/environments with a dynamic rate equal to the camera acquisition rate.


%The event-driven paradigm represents a new approach to computation and perception that aims at mimicking biological sensing systems.
%Event cameras are a recent technology that output single \textit{events} only when and where there is a change in the scene, as the intensity of light falling on the pixel changes. 
%A single events is composed by the $(x, y)$ pixel coordinates at which the change happened, a timestamp $t$ and a polarity $p$ identifying if the light has increased or decreased. 
%As opposed to the ``frame-based'' technologies, that continuously scan the entire array of pixels at a fixed rate, the asynchronous output of this cameras allows for very high temporal resolution, with latency in the order of 15 $\mu s$, and a dynamic range higher than 120 dB \cite{ATIS}. As the integration of light is not constrained to a fixed time period, artifacts due to camera motion, i.e. motion-blur, can be avoided. The amount of data produced by the sensor is strictly related to the dynamics of the scene: rapid movements generate a high number of events, ensuring the entire trajectory is represented in data, while slow movements generate less events, avoiding data redundancy.


% In \cite{ed_steering_prediction} the forecasting of an autonomous car steering angle has been addressed with event-based vision using classical deep learning methods and creating frames from the temporal integration of events. 
%How perception latency depends from task constraints and the device used - mono/stereo frame systems or mono event cameras - has been studied in \cite{how_fast_too_fast}.
% In \cite{visual_inertial_odometry} the authors aimed at estimating the position of the vision sensor in space, parametrizing the trajectory by means of B-splines. An optimization process has been performed to predict the whole sequence by minimizing a geometrical error defined in the image plane.

%In this paper we aim at exploiting the temporal information and spatially contiguous event trace generated from an event-driven camera for a predictive task towards robot interaction with a dynamic environment. As a test case, we consider a ball bouncing in front of the iCub robot~\cite{iCub}, which is equipped with an event vision systems, towards having the robot be able to catch and play. Figure~\ref{fig:bouncingBall} shows an example of the ball trajectory and the sampled position of both a traditional ``frame-based'' camera compared to an ATIS event-camera~\cite{ATIS}. Our working hypothesis is that the spatially dense trajectory captured by the event-camera should improve the prediction capabilities of a learning system and its accuracy in both time and space. Conversely, a frame-based camera may not have the temporal resolution to accurately estimate the velocity of a target through differentiation of its position, nor be able to quickly correct an estimated trajectory when a fast acceleration occurs. Instead it may be several hundreds of milliseconds before any correction can occur.  %Conversely, with frame-based cameras the trajectory is not sampled with enough temporal resolution, especially in the last part, where the bounces are shorter, or when the ball hits a surface, and the motion dynamics might not be well reconstructed. %It is interesting to notice, indeed, that several points can be acquired when the velocity of the tracked object tends to 0 - in this case because of a physical law - but not when the trajectory change is sudden - like hitting a table or a wall.  



==> Untitled Folder/methodology.tex <==

\section{Methodology}
\label{sec:methodology}

The system is comprised of the following components:
\begin{itemize}
    \item The ATIS~\cite{ATIS} event camera on the iCub robot;
    \item A target tracker that converts raw pixel events to the center of mass of the target along the trajectory;
    \item The trajectory sub-sampling strategy: either using a \textit{fixed-rate} sample or \textit{spatial} strategy; 
    \item An LSTM network, trained to predict the future trajectory of the target.
\end{itemize}

\paragraph{The ATIS camera}
Event cameras have a number of interesting properties that make them an intriguing option for pushing the visual systems of artificial agents.
% Here we analyse the difference in the sampling strategies between standard cameras and event cameras.
Traditional cameras use a \textit{fixed-rate} sampling strategy in which all the pixels are queried for the light intensity at fixed intervals (e.g. 30 Hz). Therefore the trajectory of a target viewed with a traditional camera will correspond to different spatial positions at known time intervals, which leads to a trajectory such as in Fig.~\ref{subfig:bouncingRBG}.  For fast moving objects, fixed-rate sampling can lead to gaps in the trajectory as it is under-sampled, or motion blur.
The ATIS~\cite{ATIS} is a novel visual sensor with a resolution of $304\times240$ pixels. Each pixel produces an event when the amount of light changes beyond a threshold. Each pixel produces independent events with the following information: $< x_i,y_i,t_i,p_i >$, where $<x_i,y_i>$ is the pixel position on the sensor, $t_i$ is the time the event occurred with $\mu s$ resolution, and $p_i$ is the \textit{polarity} (whether an increase or decrease in light occurred). 
Therefore the readout is not bound by the time it takes to read the entire array. Instead pixels can emit events with a very short interval between them. The effect is that a moving target will trigger each and every pixel, consecutively, along its trajectory. The positions of target observation are triggered by a \textit{spatial} threshold (a change in pixel position), and the time at which a new observation occurs is \textit{asynchronous}.

\paragraph{Target tracking}
To simplify the input to the prediction system, the raw data from the ATIS is processed to extract the mean position of the target at any point in time. The target tracking is designed to reduced the effect of noise that could occur if the visual data is directly fed into the learning system, and focus on the effect of sampling strategies on the prediction. %A tracking algorithm is also required in complex situations in which the target is not the only part of the visual stimulus, and for this event-based trackers exist, e.g.~\cite{arren_tracker}.
In this work, we implement a simple tracker with the simplifying assumption of a single moving target, as shown in Fig.~\ref{subfig:bouncingED}. The tracker accumulates events within a region-of-interest (ROI) of size $R$, and then updates the position of the ROI based on the average position of events within it. As the events move along the trajectory, so it does their mean position and the centre of the ROI. The tracker position is taken as the new centre of the ROI and is outputted along with the timestamp: $< x_{b_i},y_{b_i},t_{b_i}>$. Initialisation is performed by setting the ROI size $R$ equal to the entire image plane on the first update, and using the standard value thereafter.


\paragraph{Sub-sampling strategy}
The high temporal resolution of the event camera allows the trajectory to be sampled for every incoming event. The raw tracker data can therefore sample at over $1kHz$, but (as proposed in this paper) this raw signal can be sub-sampled to improve efficiency without compromising accuracy. Two sub-sampling strategies are proposed: in the \textit{fixed-rate} sampling we sample the signal at fixed time intervals, taking each sample after $F$ milliseconds; in the \textit{spatial} sampling we sample the signal when the spatial coordinates change by a fixed distance, taking each sample every $D$ pixels. The event camera enables very high sampling rates for both \textit{fixed-rate} and \textit{spatial} strategies. Note that the \textit{fixed-rate} strategy is more similar to a standard camera.
% \begin{itemize}
%     \item in the \textit{fixed-rate} sampling we sample the signal at fixed time intervals, taking each sample after $F$ milliseconds;
%     \item in the \textit{spatial} sampling we sample the signal when the spatial coordinates change by a fixed distance, taking each sample every \textit{delta} $D$ pixels.
% \end{itemize} 

%=====================================================================
\begin{figure}
    \centering
    \centering
    \includegraphics[width=0.8\linewidth]{error_definition2.png}
    \caption{Spatial and temporal error component of the sequence-to-sequence error for a pair of prediction and ground truth.}
  \label{fig:error_definition}
\end{figure}
%=====================================================================


% LSTM Enc-Dec
\paragraph{The LSTM network}

%\textbf{MORE PRECISE INFO ABOUT THE ENCODER DECODER ARCHITECTURE - LAYERS, AMOUNT OF NEURONS, I HAVE REALLY KNOW IDEA OF WHAT IS GOING ON HERE AND COULDN"T REPLICATE THE SYSTEM! ALSO A PARAGRAPH TO FOCUS ON THE FACT THAT TIME IS INPUT TO THE NETWORK WITH SPATIAL-DELTA SAMPLING - E.G. WHAT IS NOVEL IN YOUR SYSTEM? HIGHLIGHT IT.}
The model used in this work is a Sequence-to-Sequence LSTM architecture \cite{seq2seq-text_transl} consisting of two separate sub-networks. The Encoder takes the input data and encodes the information in a summary vector, represented by the state of the network after the input has been fed. This output becomes the initial state vector of the Decoder, that is queried to extract the information and produce the output sequence. The decoupling between the two stages allows to input sequences with a length $w_{in}$ different from the desired output sequence length $w_{out}$. This can be useful in tasks as machine translation or where the input and output physical domains differ, possibly requiring different representations. 
%Therefore, the length of both sequences is a new hyper-parameter that must be tuned in the training phase. This makes is possible to have a short input sequence (smaller input buffer) and a long output sequence. With a smaller input sequence, but long enough to predict the output sequence accurately, the system starts predicting almost immediately, as soon as the input buffer is filled. That means that the model will be highly responsive to changes. On the other hand, having different length for both sequences make it possible to predict further using longer output sequences.
Our goal is to analyse how this architecture can be combined with event cameras for predicting the upcoming trajectory of a tracked object in an asynchronous fashion.
Commonly, RNNs are queried synchronously, limited by the working rate of devices like frame-based cameras. In our case, thanks to the event camera nature, the network can be queried asynchronously every time a new event is produced by the tracker. In such a way, not only it is exploited the information coming from previous queries, but also the temporal information contained within the events. To do so, the network is fed with a sequence comprising the spatial coordinates of the trajectory in the camera space and the time interval between the events in the sequence. 
The final outcome of the network is a prediction of the next $w_{out}$ points in space and time, which is continuously updated by querying the network for each new input. The prediction consists of future spatial coordinates and, for each point, its estimated time of arrival from the current instant. This spatio-temporal trajectory output could be helpful in robotics, allowing for accurate action planning, considering both spatial and temporal information.
The Encoder architecture considered has an input layer with 3 neurons, in order to accomodate the $(X, Y)$ spatial coordinates and the temporal interval $dT$ occurred from the previous input, and an output layer of 25 neurons. The Decoder architecture, on the contrary, consists of an input layer of 25 neurons to be initialised with the final Encoder state vector, and an output layer of 3 neurons outputting the future spatial position and its time of arrival.
The Sequence-to-Sequence model is first fed with the whole input sequence of $w_{in}$ points and, only then, the output sequence of $w_{out}$ point is generated at the same time.  

==> Untitled Folder/root.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%2345678901234567890123456789012345678901234567890123456789012345678901234567890
%        1         2         3         4         5         6         7         8

% \documentclass[letterpaper, 10 pt, conference]{ieeeconf}

\IEEEoverridecommandlockouts                              % This command is only needed if 
   % you want to use the \thanks command

\overrideIEEEmargins                                      % Needed to meet printer requirements.

% See the \addtolength command later in the file to balance the column lengths
% on the last page of the document

% The following packages can be found on http:\\www.ctan.org
\usepackage{graphics} % for pdf, bitmapped graphics files
\usepackage{epsfig} % for postscript graphics files
\usepackage{mathptmx} % assumes new font selection scheme installed
\usepackage{times} % assumes new font selection scheme installed
\usepackage{amsmath} % assumes amsmath package installed
\usepackage{amssymb}  % assumes amsmath package installed

\title{\LARGE \bf
Preparation of Papers for IEEE Sponsored Conferences \& Symposia*
}


\author{Albert Author$^{1}$ and Bernard D. Researcher$^{2}$% <-this % stops a space
\thanks{*This work was not supported by any organization}% <-this % stops a space
\thanks{$^{1}$Albert Author is with Faculty of Electrical Engineering, Mathematics and Computer Science,
        University of Twente, 7500 AE Enschede, The Netherlands
        {\tt\small albert.author@papercept.net}}%
\thanks{$^{2}$Bernard D. Researcheris with the Department of Electrical Engineering, Wright State University,
        Dayton, OH 45435, USA
        {\tt\small b.d.researcher@ieee.org}}%
}


\begin{document}



\maketitle
\thispagestyle{empty}
\pagestyle{empty}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{abstract}

This electronic document is a `live' template. The various components of your paper [title, text, heads, etc.] are already defined on the style sheet, as illustrated by the portions given in this document.

\end{abstract}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{INTRODUCTION}

This template provides authors with most of the formatting specifications needed for preparing electronic versions of their papers. All standard paper components have been specified for three reasons: (1) ease of use when formatting individual papers, (2) automatic compliance to electronic requirements that facilitate the concurrent or later production of electronic products, and (3) conformity of style throughout a conference proceedings. Margins, column widths, line spacing, and type styles are built-in; examples of the type styles are provided throughout this document and are identified in italic type, within parentheses, following the example. Some components, such as multi-leveled equations, graphics, and tables are not prescribed, although the various table text styles are provided. The formatter will need to create these components, incorporating the applicable criteria that follow.

\section{PROCEDURE FOR PAPER SUBMISSION}

\subsection{Selecting a Template (Heading 2)}

First, confirm that you have the correct template for your paper size. This template has been tailored for output on the US-letter paper size. 
It may be used for A4 paper size if the paper size setting is suitably modified.

\subsection{Maintaining the Integrity of the Specifications}

The template is used to format your paper and style the text. All margins, column widths, line spaces, and text fonts are prescribed; please do not alter them. You may note peculiarities. For example, the head margin in this template measures proportionately more than is customary. This measurement and others are deliberate, using specifications that anticipate your paper as one part of the entire proceedings, and not as an independent document. Please do not revise any of the current designations

\section{MATH}

Before you begin to format your paper, first write and save the content as a separate text file. Keep your text and graphic files separate until after the text has been formatted and styled. Do not use hard tabs, and limit use of hard returns to only one return at the end of a paragraph. Do not add any kind of pagination anywhere in the paper. Do not number text heads-the template will do that for you.

Finally, complete content and organizational editing before formatting. Please take note of the following items when proofreading spelling and grammar:

\subsection{Abbreviations and Acronyms} Define abbreviations and acronyms the first time they are used in the text, even after they have been defined in the abstract. Abbreviations such as IEEE, SI, MKS, CGS, sc, dc, and rms do not have to be defined. Do not use abbreviations in the title or heads unless they are unavoidable.

\subsection{Units}

\begin{itemize}

\item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as `3.5-inch disk drive'.
\item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
\item Do not mix complete spellings and abbreviations of units: `Wb/m2' or `webers per square meter', not `webers/m2'.  Spell out units when they appear in text: `. . . a few henries', not `. . . a few H'.
\item Use a zero before decimal points: `0.25', not `.25'. Use `cm3', not `cc'. (bullet list)

\end{itemize}


\subsection{Equations}

The equations are an exception to the prescribed specifications of this template. You will need to determine whether or not your equation should be typed using either the Times New Roman or the Symbol font (please no other font). To create multileveled equations, it may be necessary to treat the equation as a graphic and insert it into the text after your paper is styled. Number equations consecutively. Equation numbers, within parentheses, are to position flush right, as in (1), using a right tab stop. To make your equations more compact, you may use the solidus ( / ), the exp function, or appropriate exponents. Italicize Roman symbols for quantities and variables, but not Greek symbols. Use a long dash rather than a hyphen for a minus sign. Punctuate equations with commas or periods when they are part of a sentence, as in

$$
\alpha + \beta = \chi \eqno{(1)}
$$

Note that the equation is centered using a center tab stop. Be sure that the symbols in your equation have been defined before or immediately following the equation. Use `(1)', not `Eq. (1)' or `equation (1)', except at the beginning of a sentence: `Equation (1) is . . .'

\subsection{Some Common Mistakes}
\begin{itemize}
\item The word `data' is plural, not singular.
\item The subscript for the permeability of vacuum 0, and other common scientific constants, is zero with subscript formatting, not a lowercase letter `o'.
\item In American English, commas, semi-/colons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is `d, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
\item A graph within a graph is an `inset', not an `insert'. The word alternatively is preferred to the word `alternately' (unless you really mean something that alternates).
\item Do not use the word `essentially' to mean `approximately' or `effectively'.
\item In your paper title, if the words `that uses' can accurately replace the word `using', capitalize the `u'; if not, keep using lower-cased.
\item Be aware of the different meanings of the homophones `affect' and `effect', `complement' and `compliment', `discreet' and `discrete', `principal' and `principle'.
\item Do not confuse `imply' and `infer'.
\item The prefix `non' is not a word; it should be joined to the word it modifies, usually without a hyphen.
\item There is no period after the `et' in the Latin abbreviation `et al.'.
\item The abbreviation `i.e.' means `that is', and the abbreviation `e.g.' means `for example'.

\end{itemize}


\section{USING THE TEMPLATE}

Use this sample document as your LaTeX source file to create your document. Save this file as {\bf root.tex}. You have to make sure to use the cls file that came with this distribution. If you use a different style file, you cannot expect to get required margins. Note also that when you are creating your out PDF file, the source file is only part of the equation. {\it Your \TeX\ $\rightarrow$ PDF filter determines the output file size. Even if you make all the specifications to output a letter file in the source - if your filter is set to produce A4, you will only get A4 output. }

It is impossible to account for all possible situation, one would encounter using \TeX. If you are using multiple \TeX\ files you must make sure that the ``MAIN`` source file is called root.tex - this is particularly important if your conference is using PaperPlaza's built in \TeX\ to PDF conversion tool.

\subsection{Headings, etc}

Text heads organize the topics on a relational, hierarchical basis. For example, the paper title is the primary text head because all subsequent material relates and elaborates on this one topic. If there are two or more sub-topics, the next level head (uppercase Roman numerals) should be used and, conversely, if there are not at least two sub-topics, then no subheads should be introduced. Styles named `Heading 1', `Heading 2', `Heading 3', and `Heading 4' are prescribed.

\subsection{Figures and Tables}

Positioning Figures and Tables: Place figures and tables at the top and bottom of columns. Avoid placing them in the middle of columns. Large figures and tables may span across both columns. Figure captions should be below the figures; table heads should appear above the tables. Insert figures and tables after they are `d in the text. Use the abbreviation `Fig. 1', even at the beginning of a sentence.

\begin{table}[h]
\caption{An Example of a Table}
\label{table_example}
\begin{center}
\begin{tabular}{|c||c|}
\hline
One & Two\\
\hline
Three & Four\\
\hline
\end{tabular}
\end{center}
\end{table}


   \begin{figure}[thpb]
      \centering
      \framebox{\parbox{3in}{We suggest that you use a text box to insert a graphic (which is ideally a 300 dpi TIFF or EPS file, with all fonts embedded) because, in an document, this method is somewhat more stable than directly inserting a picture.
}}
      %\includegraphics[scale=1.0]{figurefile}
      \caption{Inductance of oscillation winding on amorphous
       magnetic core versus DC bias magnetic field}
      \label{figurelabel}
   \end{figure}
   

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words rather than symbols or abbreviations when writing Figure axis labels to avoid confusing the reader. As an example, write the quantity `Magnetization', or `Magnetization, M', not just `M'. If including units in the label, present them within parentheses. Do not label axes only with units. In the example, write `Magnetization (A/m)' or `Magnetization {A[m(1)]}', not just `A/m'. Do not label axes with a ratio of quantities and units. For example, write `Temperature (K)', not `Temperature/K.'

\section{CONCLUSIONS}

A conclusion section is not required. Although a conclusion may review the main points of the paper, do not replicate the abstract as the conclusion. A conclusion might elaborate on the importance of the work or suggest applications and extensions. 

\addtolength{\textheight}{-12cm}   % This command serves to balance the column lengths
                                  % on the last page of the document manually. It shortens
                                  % the textheight of the last page by a suitable amount.
                                  % This command does not take effect until the next page
                                  % so it should come on the page before the last. Make
                                  % sure that you do not shorten the textheight too much.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{APPENDIX}

Appendixes should appear before the acknowledgment.

\section*{ACKNOWLEDGMENT}

The preferred spelling of the word `acknowledgment' in America is without an `e' after the `g'. Avoid the stilted expression, `One of us (R. B. G.) thanks . . .'  Instead, try `R. B. G. thanks'. Put sponsor acknowledgments in the unnumbered footnote on the first page.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

References are important to the reader; therefore, each citation must be complete and correct. If at all possible, references should be commonly available publications.
They are cited like so: \cite{IEEEexample:articleetal}, \cite{IEEEexample:book}, \cite{IEEEexample:techreptype}...



\bibliographystyle{IEEEtran}
\bibliography{IEEEabrv,IEEEexample}

\end{document}


==> Untitled Folder/template/root.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%2345678901234567890123456789012345678901234567890123456789012345678901234567890
%        1         2         3         4         5         6         7         8

% \documentclass[letterpaper, 10 pt, conference]{ieeeconf}

\IEEEoverridecommandlockouts                              % This command is only needed if 
   % you want to use the \thanks command

\overrideIEEEmargins                                      % Needed to meet printer requirements.

% See the \addtolength command later in the file to balance the column lengths
% on the last page of the document

% The following packages can be found on http:\\www.ctan.org
\usepackage{graphics} % for pdf, bitmapped graphics files
\usepackage{epsfig} % for postscript graphics files
\usepackage{mathptmx} % assumes new font selection scheme installed
\usepackage{times} % assumes new font selection scheme installed
\usepackage{amsmath} % assumes amsmath package installed
\usepackage{amssymb}  % assumes amsmath package installed

\title{\LARGE \bf
Preparation of Papers for IEEE Sponsored Conferences \& Symposia*
}


\author{Albert Author$^{1}$ and Bernard D. Researcher$^{2}$% <-this % stops a space
\thanks{*This work was not supported by any organization}% <-this % stops a space
\thanks{$^{1}$Albert Author is with Faculty of Electrical Engineering, Mathematics and Computer Science,
        University of Twente, 7500 AE Enschede, The Netherlands
        {\tt\small albert.author@papercept.net}}%
\thanks{$^{2}$Bernard D. Researcheris with the Department of Electrical Engineering, Wright State University,
        Dayton, OH 45435, USA
        {\tt\small b.d.researcher@ieee.org}}%
}


\begin{document}



\maketitle
\thispagestyle{empty}
\pagestyle{empty}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{abstract}

This electronic document is a `live' template. The various components of your paper [title, text, heads, etc.] are already defined on the style sheet, as illustrated by the portions given in this document.

\end{abstract}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{INTRODUCTION}

This template provides authors with most of the formatting specifications needed for preparing electronic versions of their papers. All standard paper components have been specified for three reasons: (1) ease of use when formatting individual papers, (2) automatic compliance to electronic requirements that facilitate the concurrent or later production of electronic products, and (3) conformity of style throughout a conference proceedings. Margins, column widths, line spacing, and type styles are built-in; examples of the type styles are provided throughout this document and are identified in italic type, within parentheses, following the example. Some components, such as multi-leveled equations, graphics, and tables are not prescribed, although the various table text styles are provided. The formatter will need to create these components, incorporating the applicable criteria that follow.

\section{PROCEDURE FOR PAPER SUBMISSION}

\subsection{Selecting a Template (Heading 2)}

First, confirm that you have the correct template for your paper size. This template has been tailored for output on the US-letter paper size. 
It may be used for A4 paper size if the paper size setting is suitably modified.

\subsection{Maintaining the Integrity of the Specifications}

The template is used to format your paper and style the text. All margins, column widths, line spaces, and text fonts are prescribed; please do not alter them. You may note peculiarities. For example, the head margin in this template measures proportionately more than is customary. This measurement and others are deliberate, using specifications that anticipate your paper as one part of the entire proceedings, and not as an independent document. Please do not revise any of the current designations

\section{MATH}

Before you begin to format your paper, first write and save the content as a separate text file. Keep your text and graphic files separate until after the text has been formatted and styled. Do not use hard tabs, and limit use of hard returns to only one return at the end of a paragraph. Do not add any kind of pagination anywhere in the paper. Do not number text heads-the template will do that for you.

Finally, complete content and organizational editing before formatting. Please take note of the following items when proofreading spelling and grammar:

\subsection{Abbreviations and Acronyms} Define abbreviations and acronyms the first time they are used in the text, even after they have been defined in the abstract. Abbreviations such as IEEE, SI, MKS, CGS, sc, dc, and rms do not have to be defined. Do not use abbreviations in the title or heads unless they are unavoidable.

\subsection{Units}

\begin{itemize}

\item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as `3.5-inch disk drive'.
\item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
\item Do not mix complete spellings and abbreviations of units: `Wb/m2' or `webers per square meter', not `webers/m2'.  Spell out units when they appear in text: `. . . a few henries', not `. . . a few H'.
\item Use a zero before decimal points: `0.25', not `.25'. Use `cm3', not `cc'. (bullet list)

\end{itemize}


\subsection{Equations}

The equations are an exception to the prescribed specifications of this template. You will need to determine whether or not your equation should be typed using either the Times New Roman or the Symbol font (please no other font). To create multileveled equations, it may be necessary to treat the equation as a graphic and insert it into the text after your paper is styled. Number equations consecutively. Equation numbers, within parentheses, are to position flush right, as in (1), using a right tab stop. To make your equations more compact, you may use the solidus ( / ), the exp function, or appropriate exponents. Italicize Roman symbols for quantities and variables, but not Greek symbols. Use a long dash rather than a hyphen for a minus sign. Punctuate equations with commas or periods when they are part of a sentence, as in

$$
\alpha + \beta = \chi \eqno{(1)}
$$

Note that the equation is centered using a center tab stop. Be sure that the symbols in your equation have been defined before or immediately following the equation. Use `(1)', not `Eq. (1)' or `equation (1)', except at the beginning of a sentence: `Equation (1) is . . .'

\subsection{Some Common Mistakes}
\begin{itemize}
\item The word `data' is plural, not singular.
\item The subscript for the permeability of vacuum 0, and other common scientific constants, is zero with subscript formatting, not a lowercase letter `o'.
\item In American English, commas, semi-/colons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is `d, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
\item A graph within a graph is an `inset', not an `insert'. The word alternatively is preferred to the word `alternately' (unless you really mean something that alternates).
\item Do not use the word `essentially' to mean `approximately' or `effectively'.
\item In your paper title, if the words `that uses' can accurately replace the word `using', capitalize the `u'; if not, keep using lower-cased.
\item Be aware of the different meanings of the homophones `affect' and `effect', `complement' and `compliment', `discreet' and `discrete', `principal' and `principle'.
\item Do not confuse `imply' and `infer'.
\item The prefix `non' is not a word; it should be joined to the word it modifies, usually without a hyphen.
\item There is no period after the `et' in the Latin abbreviation `et al.'.
\item The abbreviation `i.e.' means `that is', and the abbreviation `e.g.' means `for example'.

\end{itemize}


\section{USING THE TEMPLATE}

Use this sample document as your LaTeX source file to create your document. Save this file as {\bf root.tex}. You have to make sure to use the cls file that came with this distribution. If you use a different style file, you cannot expect to get required margins. Note also that when you are creating your out PDF file, the source file is only part of the equation. {\it Your \TeX\ $\rightarrow$ PDF filter determines the output file size. Even if you make all the specifications to output a letter file in the source - if your filter is set to produce A4, you will only get A4 output. }

It is impossible to account for all possible situation, one would encounter using \TeX. If you are using multiple \TeX\ files you must make sure that the ``MAIN`` source file is called root.tex - this is particularly important if your conference is using PaperPlaza's built in \TeX\ to PDF conversion tool.

\subsection{Headings, etc}

Text heads organize the topics on a relational, hierarchical basis. For example, the paper title is the primary text head because all subsequent material relates and elaborates on this one topic. If there are two or more sub-topics, the next level head (uppercase Roman numerals) should be used and, conversely, if there are not at least two sub-topics, then no subheads should be introduced. Styles named `Heading 1', `Heading 2', `Heading 3', and `Heading 4' are prescribed.

\subsection{Figures and Tables}

Positioning Figures and Tables: Place figures and tables at the top and bottom of columns. Avoid placing them in the middle of columns. Large figures and tables may span across both columns. Figure captions should be below the figures; table heads should appear above the tables. Insert figures and tables after they are `d in the text. Use the abbreviation `Fig. 1', even at the beginning of a sentence.

\begin{table}[h]
\caption{An Example of a Table}
\label{table_example}
\begin{center}
\begin{tabular}{|c||c|}
\hline
One & Two\\
\hline
Three & Four\\
\hline
\end{tabular}
\end{center}
\end{table}


   \begin{figure}[thpb]
      \centering
      \framebox{\parbox{3in}{We suggest that you use a text box to insert a graphic (which is ideally a 300 dpi TIFF or EPS file, with all fonts embedded) because, in an document, this method is somewhat more stable than directly inserting a picture.
}}
      %\includegraphics[scale=1.0]{figurefile}
      \caption{Inductance of oscillation winding on amorphous
       magnetic core versus DC bias magnetic field}
      \label{figurelabel}
   \end{figure}
   

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words rather than symbols or abbreviations when writing Figure axis labels to avoid confusing the reader. As an example, write the quantity `Magnetization', or `Magnetization, M', not just `M'. If including units in the label, present them within parentheses. Do not label axes only with units. In the example, write `Magnetization (A/m)' or `Magnetization {A[m(1)]}', not just `A/m'. Do not label axes with a ratio of quantities and units. For example, write `Temperature (K)', not `Temperature/K.'

\section{CONCLUSIONS}

A conclusion section is not required. Although a conclusion may review the main points of the paper, do not replicate the abstract as the conclusion. A conclusion might elaborate on the importance of the work or suggest applications and extensions. 

\addtolength{\textheight}{-12cm}   % This command serves to balance the column lengths
                                  % on the last page of the document manually. It shortens
                                  % the textheight of the last page by a suitable amount.
                                  % This command does not take effect until the next page
                                  % so it should come on the page before the last. Make
                                  % sure that you do not shorten the textheight too much.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{APPENDIX}

Appendixes should appear before the acknowledgment.

\section*{ACKNOWLEDGMENT}

The preferred spelling of the word `acknowledgment' in America is without an `e' after the `g'. Avoid the stilted expression, `One of us (R. B. G.) thanks . . .'  Instead, try `R. B. G. thanks'. Put sponsor acknowledgments in the unnumbered footnote on the first page.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

References are important to the reader; therefore, each citation must be complete and correct. If at all possible, references should be commonly available publications.
They are cited like so: \cite{IEEEexample:articleetal}, \cite{IEEEexample:book}, \cite{IEEEexample:techreptype}...



\bibliographystyle{IEEEtran}
\bibliography{IEEEabrv,IEEEexample}

\end{document}


==> root.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%2345678901234567890123456789012345678901234567890123456789012345678901234567890
%        1         2         3         4         5         6         7         8

% \documentclass[letterpaper, 10 pt, conference]{ieeeconf}

\IEEEoverridecommandlockouts                              % This command is only needed if 
   % you want to use the \thanks command

\overrideIEEEmargins                                      % Needed to meet printer requirements.

% See the \addtolength command later in the file to balance the column lengths
% on the last page of the document

% The following packages can be found on http:\\www.ctan.org
\usepackage{graphics} % for pdf, bitmapped graphics files
\usepackage{epsfig} % for postscript graphics files
\usepackage{mathptmx} % assumes new font selection scheme installed
\usepackage{times} % assumes new font selection scheme installed
\usepackage{amsmath} % assumes amsmath package installed
\usepackage{amssymb}  % assumes amsmath package installed

\title{\LARGE \bf
Preparation of Papers for IEEE Sponsored Conferences \& Symposia*
}


\author{Albert Author$^{1}$ and Bernard D. Researcher$^{2}$% <-this % stops a space
\thanks{*This work was not supported by any organization}% <-this % stops a space
\thanks{$^{1}$Albert Author is with Faculty of Electrical Engineering, Mathematics and Computer Science,
        University of Twente, 7500 AE Enschede, The Netherlands
        {\tt\small albert.author@papercept.net}}%
\thanks{$^{2}$Bernard D. Researcheris with the Department of Electrical Engineering, Wright State University,
        Dayton, OH 45435, USA
        {\tt\small b.d.researcher@ieee.org}}%
}


\begin{document}



\maketitle
\thispagestyle{empty}
\pagestyle{empty}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{abstract}

This electronic document is a `live' template. The various components of your paper [title, text, heads, etc.] are already defined on the style sheet, as illustrated by the portions given in this document.

\end{abstract}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{INTRODUCTION}

This template provides authors with most of the formatting specifications needed for preparing electronic versions of their papers. All standard paper components have been specified for three reasons: (1) ease of use when formatting individual papers, (2) automatic compliance to electronic requirements that facilitate the concurrent or later production of electronic products, and (3) conformity of style throughout a conference proceedings. Margins, column widths, line spacing, and type styles are built-in; examples of the type styles are provided throughout this document and are identified in italic type, within parentheses, following the example. Some components, such as multi-leveled equations, graphics, and tables are not prescribed, although the various table text styles are provided. The formatter will need to create these components, incorporating the applicable criteria that follow.

\section{PROCEDURE FOR PAPER SUBMISSION}

\subsection{Selecting a Template (Heading 2)}

First, confirm that you have the correct template for your paper size. This template has been tailored for output on the US-letter paper size. 
It may be used for A4 paper size if the paper size setting is suitably modified.

\subsection{Maintaining the Integrity of the Specifications}

The template is used to format your paper and style the text. All margins, column widths, line spaces, and text fonts are prescribed; please do not alter them. You may note peculiarities. For example, the head margin in this template measures proportionately more than is customary. This measurement and others are deliberate, using specifications that anticipate your paper as one part of the entire proceedings, and not as an independent document. Please do not revise any of the current designations

\section{MATH}

Before you begin to format your paper, first write and save the content as a separate text file. Keep your text and graphic files separate until after the text has been formatted and styled. Do not use hard tabs, and limit use of hard returns to only one return at the end of a paragraph. Do not add any kind of pagination anywhere in the paper. Do not number text heads-the template will do that for you.

Finally, complete content and organizational editing before formatting. Please take note of the following items when proofreading spelling and grammar:

\subsection{Abbreviations and Acronyms} Define abbreviations and acronyms the first time they are used in the text, even after they have been defined in the abstract. Abbreviations such as IEEE, SI, MKS, CGS, sc, dc, and rms do not have to be defined. Do not use abbreviations in the title or heads unless they are unavoidable.

\subsection{Units}

\begin{itemize}

\item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as `3.5-inch disk drive'.
\item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
\item Do not mix complete spellings and abbreviations of units: `Wb/m2' or `webers per square meter', not `webers/m2'.  Spell out units when they appear in text: `. . . a few henries', not `. . . a few H'.
\item Use a zero before decimal points: `0.25', not `.25'. Use `cm3', not `cc'. (bullet list)

\end{itemize}


\subsection{Equations}

The equations are an exception to the prescribed specifications of this template. You will need to determine whether or not your equation should be typed using either the Times New Roman or the Symbol font (please no other font). To create multileveled equations, it may be necessary to treat the equation as a graphic and insert it into the text after your paper is styled. Number equations consecutively. Equation numbers, within parentheses, are to position flush right, as in (1), using a right tab stop. To make your equations more compact, you may use the solidus ( / ), the exp function, or appropriate exponents. Italicize Roman symbols for quantities and variables, but not Greek symbols. Use a long dash rather than a hyphen for a minus sign. Punctuate equations with commas or periods when they are part of a sentence, as in

$$
\alpha + \beta = \chi \eqno{(1)}
$$

Note that the equation is centered using a center tab stop. Be sure that the symbols in your equation have been defined before or immediately following the equation. Use `(1)', not `Eq. (1)' or `equation (1)', except at the beginning of a sentence: `Equation (1) is . . .'

\subsection{Some Common Mistakes}
\begin{itemize}
\item The word `data' is plural, not singular.
\item The subscript for the permeability of vacuum 0, and other common scientific constants, is zero with subscript formatting, not a lowercase letter `o'.
\item In American English, commas, semi-/colons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is `d, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
\item A graph within a graph is an `inset', not an `insert'. The word alternatively is preferred to the word `alternately' (unless you really mean something that alternates).
\item Do not use the word `essentially' to mean `approximately' or `effectively'.
\item In your paper title, if the words `that uses' can accurately replace the word `using', capitalize the `u'; if not, keep using lower-cased.
\item Be aware of the different meanings of the homophones `affect' and `effect', `complement' and `compliment', `discreet' and `discrete', `principal' and `principle'.
\item Do not confuse `imply' and `infer'.
\item The prefix `non' is not a word; it should be joined to the word it modifies, usually without a hyphen.
\item There is no period after the `et' in the Latin abbreviation `et al.'.
\item The abbreviation `i.e.' means `that is', and the abbreviation `e.g.' means `for example'.

\end{itemize}


\section{USING THE TEMPLATE}

Use this sample document as your LaTeX source file to create your document. Save this file as {\bf root.tex}. You have to make sure to use the cls file that came with this distribution. If you use a different style file, you cannot expect to get required margins. Note also that when you are creating your out PDF file, the source file is only part of the equation. {\it Your \TeX\ $\rightarrow$ PDF filter determines the output file size. Even if you make all the specifications to output a letter file in the source - if your filter is set to produce A4, you will only get A4 output. }

It is impossible to account for all possible situation, one would encounter using \TeX. If you are using multiple \TeX\ files you must make sure that the ``MAIN`` source file is called root.tex - this is particularly important if your conference is using PaperPlaza's built in \TeX\ to PDF conversion tool.

\subsection{Headings, etc}

Text heads organize the topics on a relational, hierarchical basis. For example, the paper title is the primary text head because all subsequent material relates and elaborates on this one topic. If there are two or more sub-topics, the next level head (uppercase Roman numerals) should be used and, conversely, if there are not at least two sub-topics, then no subheads should be introduced. Styles named `Heading 1', `Heading 2', `Heading 3', and `Heading 4' are prescribed.

\subsection{Figures and Tables}

Positioning Figures and Tables: Place figures and tables at the top and bottom of columns. Avoid placing them in the middle of columns. Large figures and tables may span across both columns. Figure captions should be below the figures; table heads should appear above the tables. Insert figures and tables after they are `d in the text. Use the abbreviation `Fig. 1', even at the beginning of a sentence.

\begin{table}[h]
\caption{An Example of a Table}
\label{table_example}
\begin{center}
\begin{tabular}{|c||c|}
\hline
One & Two\\
\hline
Three & Four\\
\hline
\end{tabular}
\end{center}
\end{table}


   \begin{figure}[thpb]
      \centering
      \framebox{\parbox{3in}{We suggest that you use a text box to insert a graphic (which is ideally a 300 dpi TIFF or EPS file, with all fonts embedded) because, in an document, this method is somewhat more stable than directly inserting a picture.
}}
      %\includegraphics[scale=1.0]{figurefile}
      \caption{Inductance of oscillation winding on amorphous
       magnetic core versus DC bias magnetic field}
      \label{figurelabel}
   \end{figure}
   

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words rather than symbols or abbreviations when writing Figure axis labels to avoid confusing the reader. As an example, write the quantity `Magnetization', or `Magnetization, M', not just `M'. If including units in the label, present them within parentheses. Do not label axes only with units. In the example, write `Magnetization (A/m)' or `Magnetization {A[m(1)]}', not just `A/m'. Do not label axes with a ratio of quantities and units. For example, write `Temperature (K)', not `Temperature/K.'

\section{CONCLUSIONS}

A conclusion section is not required. Although a conclusion may review the main points of the paper, do not replicate the abstract as the conclusion. A conclusion might elaborate on the importance of the work or suggest applications and extensions. 

\addtolength{\textheight}{-12cm}   % This command serves to balance the column lengths
                                  % on the last page of the document manually. It shortens
                                  % the textheight of the last page by a suitable amount.
                                  % This command does not take effect until the next page
                                  % so it should come on the page before the last. Make
                                  % sure that you do not shorten the textheight too much.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{APPENDIX}

Appendixes should appear before the acknowledgment.

\section*{ACKNOWLEDGMENT}

The preferred spelling of the word `acknowledgment' in America is without an `e' after the `g'. Avoid the stilted expression, `One of us (R. B. G.) thanks . . .'  Instead, try `R. B. G. thanks'. Put sponsor acknowledgments in the unnumbered footnote on the first page.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

References are important to the reader; therefore, each citation must be complete and correct. If at all possible, references should be commonly available publications.
They are cited like so: \cite{IEEEexample:articleetal}, \cite{IEEEexample:book}, \cite{IEEEexample:techreptype}...



\bibliographystyle{IEEEtran}
\bibliography{IEEEabrv,IEEEexample}

\end{document}


==> template/root.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%2345678901234567890123456789012345678901234567890123456789012345678901234567890
%        1         2         3         4         5         6         7         8

% \documentclass[letterpaper, 10 pt, conference]{ieeeconf}

\IEEEoverridecommandlockouts                              % This command is only needed if 
   % you want to use the \thanks command

\overrideIEEEmargins                                      % Needed to meet printer requirements.

% See the \addtolength command later in the file to balance the column lengths
% on the last page of the document

% The following packages can be found on http:\\www.ctan.org
\usepackage{graphics} % for pdf, bitmapped graphics files
\usepackage{epsfig} % for postscript graphics files
\usepackage{mathptmx} % assumes new font selection scheme installed
\usepackage{times} % assumes new font selection scheme installed
\usepackage{amsmath} % assumes amsmath package installed
\usepackage{amssymb}  % assumes amsmath package installed

\title{\LARGE \bf
Preparation of Papers for IEEE Sponsored Conferences \& Symposia*
}


\author{Albert Author$^{1}$ and Bernard D. Researcher$^{2}$% <-this % stops a space
\thanks{*This work was not supported by any organization}% <-this % stops a space
\thanks{$^{1}$Albert Author is with Faculty of Electrical Engineering, Mathematics and Computer Science,
        University of Twente, 7500 AE Enschede, The Netherlands
        {\tt\small albert.author@papercept.net}}%
\thanks{$^{2}$Bernard D. Researcheris with the Department of Electrical Engineering, Wright State University,
        Dayton, OH 45435, USA
        {\tt\small b.d.researcher@ieee.org}}%
}


\begin{document}



\maketitle
\thispagestyle{empty}
\pagestyle{empty}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{abstract}

This electronic document is a `live' template. The various components of your paper [title, text, heads, etc.] are already defined on the style sheet, as illustrated by the portions given in this document.

\end{abstract}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{INTRODUCTION}

This template provides authors with most of the formatting specifications needed for preparing electronic versions of their papers. All standard paper components have been specified for three reasons: (1) ease of use when formatting individual papers, (2) automatic compliance to electronic requirements that facilitate the concurrent or later production of electronic products, and (3) conformity of style throughout a conference proceedings. Margins, column widths, line spacing, and type styles are built-in; examples of the type styles are provided throughout this document and are identified in italic type, within parentheses, following the example. Some components, such as multi-leveled equations, graphics, and tables are not prescribed, although the various table text styles are provided. The formatter will need to create these components, incorporating the applicable criteria that follow.

\section{PROCEDURE FOR PAPER SUBMISSION}

\subsection{Selecting a Template (Heading 2)}

First, confirm that you have the correct template for your paper size. This template has been tailored for output on the US-letter paper size. 
It may be used for A4 paper size if the paper size setting is suitably modified.

\subsection{Maintaining the Integrity of the Specifications}

The template is used to format your paper and style the text. All margins, column widths, line spaces, and text fonts are prescribed; please do not alter them. You may note peculiarities. For example, the head margin in this template measures proportionately more than is customary. This measurement and others are deliberate, using specifications that anticipate your paper as one part of the entire proceedings, and not as an independent document. Please do not revise any of the current designations

\section{MATH}

Before you begin to format your paper, first write and save the content as a separate text file. Keep your text and graphic files separate until after the text has been formatted and styled. Do not use hard tabs, and limit use of hard returns to only one return at the end of a paragraph. Do not add any kind of pagination anywhere in the paper. Do not number text heads-the template will do that for you.

Finally, complete content and organizational editing before formatting. Please take note of the following items when proofreading spelling and grammar:

\subsection{Abbreviations and Acronyms} Define abbreviations and acronyms the first time they are used in the text, even after they have been defined in the abstract. Abbreviations such as IEEE, SI, MKS, CGS, sc, dc, and rms do not have to be defined. Do not use abbreviations in the title or heads unless they are unavoidable.

\subsection{Units}

\begin{itemize}

\item Use either SI (MKS) or CGS as primary units. (SI units are encouraged.) English units may be used as secondary units (in parentheses). An exception would be the use of English units as identifiers in trade, such as `3.5-inch disk drive'.
\item Avoid combining SI and CGS units, such as current in amperes and magnetic field in oersteds. This often leads to confusion because equations do not balance dimensionally. If you must use mixed units, clearly state the units for each quantity that you use in an equation.
\item Do not mix complete spellings and abbreviations of units: `Wb/m2' or `webers per square meter', not `webers/m2'.  Spell out units when they appear in text: `. . . a few henries', not `. . . a few H'.
\item Use a zero before decimal points: `0.25', not `.25'. Use `cm3', not `cc'. (bullet list)

\end{itemize}


\subsection{Equations}

The equations are an exception to the prescribed specifications of this template. You will need to determine whether or not your equation should be typed using either the Times New Roman or the Symbol font (please no other font). To create multileveled equations, it may be necessary to treat the equation as a graphic and insert it into the text after your paper is styled. Number equations consecutively. Equation numbers, within parentheses, are to position flush right, as in (1), using a right tab stop. To make your equations more compact, you may use the solidus ( / ), the exp function, or appropriate exponents. Italicize Roman symbols for quantities and variables, but not Greek symbols. Use a long dash rather than a hyphen for a minus sign. Punctuate equations with commas or periods when they are part of a sentence, as in

$$
\alpha + \beta = \chi \eqno{(1)}
$$

Note that the equation is centered using a center tab stop. Be sure that the symbols in your equation have been defined before or immediately following the equation. Use `(1)', not `Eq. (1)' or `equation (1)', except at the beginning of a sentence: `Equation (1) is . . .'

\subsection{Some Common Mistakes}
\begin{itemize}
\item The word `data' is plural, not singular.
\item The subscript for the permeability of vacuum 0, and other common scientific constants, is zero with subscript formatting, not a lowercase letter `o'.
\item In American English, commas, semi-/colons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is `d, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
\item A graph within a graph is an `inset', not an `insert'. The word alternatively is preferred to the word `alternately' (unless you really mean something that alternates).
\item Do not use the word `essentially' to mean `approximately' or `effectively'.
\item In your paper title, if the words `that uses' can accurately replace the word `using', capitalize the `u'; if not, keep using lower-cased.
\item Be aware of the different meanings of the homophones `affect' and `effect', `complement' and `compliment', `discreet' and `discrete', `principal' and `principle'.
\item Do not confuse `imply' and `infer'.
\item The prefix `non' is not a word; it should be joined to the word it modifies, usually without a hyphen.
\item There is no period after the `et' in the Latin abbreviation `et al.'.
\item The abbreviation `i.e.' means `that is', and the abbreviation `e.g.' means `for example'.

\end{itemize}


\section{USING THE TEMPLATE}

Use this sample document as your LaTeX source file to create your document. Save this file as {\bf root.tex}. You have to make sure to use the cls file that came with this distribution. If you use a different style file, you cannot expect to get required margins. Note also that when you are creating your out PDF file, the source file is only part of the equation. {\it Your \TeX\ $\rightarrow$ PDF filter determines the output file size. Even if you make all the specifications to output a letter file in the source - if your filter is set to produce A4, you will only get A4 output. }

It is impossible to account for all possible situation, one would encounter using \TeX. If you are using multiple \TeX\ files you must make sure that the ``MAIN`` source file is called root.tex - this is particularly important if your conference is using PaperPlaza's built in \TeX\ to PDF conversion tool.

\subsection{Headings, etc}

Text heads organize the topics on a relational, hierarchical basis. For example, the paper title is the primary text head because all subsequent material relates and elaborates on this one topic. If there are two or more sub-topics, the next level head (uppercase Roman numerals) should be used and, conversely, if there are not at least two sub-topics, then no subheads should be introduced. Styles named `Heading 1', `Heading 2', `Heading 3', and `Heading 4' are prescribed.

\subsection{Figures and Tables}

Positioning Figures and Tables: Place figures and tables at the top and bottom of columns. Avoid placing them in the middle of columns. Large figures and tables may span across both columns. Figure captions should be below the figures; table heads should appear above the tables. Insert figures and tables after they are `d in the text. Use the abbreviation `Fig. 1', even at the beginning of a sentence.

\begin{table}[h]
\caption{An Example of a Table}
\label{table_example}
\begin{center}
\begin{tabular}{|c||c|}
\hline
One & Two\\
\hline
Three & Four\\
\hline
\end{tabular}
\end{center}
\end{table}


   \begin{figure}[thpb]
      \centering
      \framebox{\parbox{3in}{We suggest that you use a text box to insert a graphic (which is ideally a 300 dpi TIFF or EPS file, with all fonts embedded) because, in an document, this method is somewhat more stable than directly inserting a picture.
}}
      %\includegraphics[scale=1.0]{figurefile}
      \caption{Inductance of oscillation winding on amorphous
       magnetic core versus DC bias magnetic field}
      \label{figurelabel}
   \end{figure}
   

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words rather than symbols or abbreviations when writing Figure axis labels to avoid confusing the reader. As an example, write the quantity `Magnetization', or `Magnetization, M', not just `M'. If including units in the label, present them within parentheses. Do not label axes only with units. In the example, write `Magnetization (A/m)' or `Magnetization {A[m(1)]}', not just `A/m'. Do not label axes with a ratio of quantities and units. For example, write `Temperature (K)', not `Temperature/K.'

\section{CONCLUSIONS}

A conclusion section is not required. Although a conclusion may review the main points of the paper, do not replicate the abstract as the conclusion. A conclusion might elaborate on the importance of the work or suggest applications and extensions. 

\addtolength{\textheight}{-12cm}   % This command serves to balance the column lengths
                                  % on the last page of the document manually. It shortens
                                  % the textheight of the last page by a suitable amount.
                                  % This command does not take effect until the next page
                                  % so it should come on the page before the last. Make
                                  % sure that you do not shorten the textheight too much.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{APPENDIX}

Appendixes should appear before the acknowledgment.

\section*{ACKNOWLEDGMENT}

The preferred spelling of the word `acknowledgment' in America is without an `e' after the `g'. Avoid the stilted expression, `One of us (R. B. G.) thanks . . .'  Instead, try `R. B. G. thanks'. Put sponsor acknowledgments in the unnumbered footnote on the first page.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

References are important to the reader; therefore, each citation must be complete and correct. If at all possible, references should be commonly available publications.
They are cited like so: \cite{IEEEexample:articleetal}, \cite{IEEEexample:book}, \cite{IEEEexample:techreptype}...



\bibliographystyle{IEEEtran}
\bibliography{IEEEabrv,IEEEexample}

\end{document}

